A Dynamical Systems Analysis of Trap Music Exposure and School Dropout Among Costa Rican Adolescents

In recent years, a surge in the popularity of trap music among adolescents has prompted concerns about its potential influence on youth behavior and educational outcomes. In this study, we develop a novel compartmental model using a system of differential equations to explore the relationship between exposure to trap music and school dropout rates among Costa Rican adolescents aged 13 to 17. The model divides the population into distinct compartments representing susceptible individuals, casual listeners, active participants, those exhibiting risk-associated behaviors, and ultimately, school dropouts. Key parameters, including transmission via peer influence, progression rates between exposure stages, and recovery dynamics, capture the complex interplay between cultural diffusion and behavioral change. Analytical investigation of the basic reproductive number, $R_0$, and both trap-free and endemic equilibrium states provide insight into the conditions under which the influence of trap music proliferates. Numerical simulations, implemented in MATLAB, further illustrate how parameter variations, especially the potential for recovery, affect the system's dynamics. Our results suggest that although exposure to trap music is widespread, the progression to adverse behavioral outcomes leading to school dropout is highly sensitive to intervention strategies, offering valuable implications for educational policy and targeted preventive measures.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk --shell-escape -pdf \"$_[0]\"" );
    }
}
